An encoder-decoder-based method for COVID-19 lung infection segmentation

The novelty of the COVID-19 disease and the speed of spread has created a colossal chaos, impulse among researchers worldwide to exploit all the resources and capabilities to understand and analyze characteristics of the coronavirus in term of the ways it spreads and virus incubation time. For that, the existing medical features like CT and X-ray images are used. For example, CT-scan images can be used for the detection of lung infection. But the challenges of these features such as the quality of the image and infection characteristics limitate the effectiveness of these features. Using artificial intelligence (AI) tools and computer vision algorithms, the accuracy of detection can be more accurate and can help to overcome these issues. This paper proposes a multi-task deep-learning-based method for lung infection segmentation using CT-scan images. Our proposed method starts by segmenting the lung regions that can be infected. Then, segmenting the infections in these regions. Also, to perform a multi-class segmentation the proposed model is trained using the two-stream inputs. The multi-task learning used in this paper allows us to overcome shortage of labeled data. Also, the multi-input stream allows the model to do the learning on many features that can improve the results. To evaluate the proposed method, many features have been used. Also, from the experiments, the proposed method can segment lung infections with a high degree performance even with shortage of data and labeled images. In addition, comparing with the state-of-the-art method our method achieves good performance results.

==> arcxiv tex/references.tex <==
\begin{thebibliography}{00}

 \bibitem{1}     F. Porikli, F. Br´emond, S. L. Dockstader, J. Ferryman, A. Hoogs, B. C.
Lovell, S. Pankanti, B. Rinner, P. Tu, P. L. Venetianer, Video surveillance:
 past, present, and now the future [dsp forum}, IEEE Signal Processing
Magazine 30 (3) (2013) 190\-198.

 \bibitem{2} D. Cumming, S. Johan, Cameras tracking shoppers: the economics of
retail video surveillance, Eurasian Business Review 5 (2) (2015) 235\-257.

 \bibitem{3} Y. Tang, B. Ma, H. Yan, Intelligent video surveillance system for elderly
 people living alone based on odvs, Advances in Internet of Things 3 (02)
(2013)

 \bibitem{4} J. M. Such, A. Espinosa, A. Garc´ıa-Fornes, A survey of privacy in multiagent systems, The Knowledge Engineering Review 29 (3) (2014) 314\-344.

 \bibitem{5} M. Cristani, R. Raghavendra, A. Del Bue, V. Murino, Human behav-
 ior analysis in video surveillance: A social signal processing perspective,
Neurocomputing 100 (2013) 86\-97.
 \bibitem{6} A. G. Bole, W. O. Dineley, A. Wall, Radar and ARPA manual, Elsevier
Butterworth Heinemann, 2005.

 \bibitem{7} J. Lubczonek, A. Stateczny, Aspects of spatial planning of radar sensor
 network for inland waterways surveillance, in: Radar Conference, 2009.
EuRAD 2009. European, IEEE, 2009, pp. 501\-504.
 \bibitem{8} A. Borkowski, Filtering of aerial laser scanning data by active surface
model, Annals of Geomatics 2006 3 (4).

 \bibitem{9} R. T. Collins, A. J. Lipton, T. Kanade, Introduction to the special section
 on video surveillance, IEEE Transactions on pattern analysis and machine
intelligence 22 (8) (2000) 745\-746.

 \bibitem{10} Z. Xu, Y. Liu, L. Mei, C. Hu, L. Chen, Semantic based representing
and organizing surveillance big data using video structural description
technology, Journal of Systems and Software 102 (2015) 217\-225.

  \item \relax  [11} Z. Xu, C. Hu, L. Mei, Video structured description technology based
intelligence analysis of surveillance videos for public security applications,
Multimedia Tools and Applications 75 (19) (2016) 12155\-12172.

 \bibitem{12} O. El Harrouss, D. Moujahid, H. Tairi, Motion detection based on the
combining of the background subtraction and spatial color information,
 in: Intelligent Systems and Computer Vision (ISCV), 2015, IEEE, 2015,
pp. 1\-4.

 \bibitem{13} S. Khokhar, I. Saleemi, M. Shah, Multi-agent event recognition by preservation of spatiotemporal relationships between probabilistic models, Image and Vision Computing 31 (9) (2013) 603\-615.

  \item \relax  [14} H. Wang, A. Kl¨aser, C. Schmid, C.-L. Liu, Dense trajectories and motion boundary descriptors for action recognition, International journal of
computer vision 103 (1) (2013) 60\-79.

 \bibitem{15} H. Wang, C. Yuan, W. Hu, H. Ling, W. Yang, C. Sun, Action recognition using nonnegative action component representation and sparse basis
 selection, IEEE transactions on image processing 23 (2) (2014) 570\-581.
 
 \bibitem{16} T. E. Boult, R. J. Micheals, X. Gao, M. Eckmann, Into the woods: Visual surveillance of noncooperative and camouflaged targets in complex
outdoor settings, Proceedings of the IEEE 89 (10) (2001) 1382\-1402.

 \bibitem{17} C. P. Diehl, Toward efficient collaborative classification for distributed
 video surveillance, Ph.D. thesis, Citeseer (2000).
 
 \item \relax [18} D. M. Gavrila, The visual analysis of human movement: A survey, Computer vision and image understanding 73 (1) (1999) 82\-98.

 \bibitem{19} J. Templer, J. Archea, H. H. Chen, Study of factors associated with risk
of work-related stairway falls, Journal of Safety Research 16 (4) (1985)
 183\-196.
 \bibitem{20} T. Cav´en, J. Saari, Videotape-based interviews in safety analysis, Journal
of Occupational Accidents 4 (2-4) (1982) 341\-345.

 \bibitem{21} P. Cocca, F. Marciano, D. Rossi, Assessment of biomechanical risk at
work: practical approaches and tools, Acta of bioengineering and biome-
 chanics 10 (3) (2008) 21\-27.
 
 \bibitem{22} G. David, Ergonomic methods for assessing exposure to risk factors
for work-related musculoskeletal disorders, Occupational medicine 55 (3)
(2005) 190\-99.

 \bibitem{23} G. L. Foresti, P. Mahonen, C. S. Regazzoni, Multimedia video-based
 surveillance systems: Requirements, Issues and Solutions, Vol. 573,
Springer Science \& Business Media, 2012.
 \bibitem{24} P. Natarajan, P. K. Atrey, M. Kankanhalli, Multi-camera coordination
and control in surveillance systems: A survey, ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM) 11 (4)
 (2015) 57.
 \bibitem{25} D. Stepanov, I. Tishchenko, The concept of video surveillance system
based on the principles of stereo vision., in: FRUCT, 2016, pp. 328\-334.

 \bibitem{26} P. Corke, T. Wark, R. Jurdak, W. Hu, P. Valencia, D. Moore, Environmental wireless sensor networks, Proceedings of the IEEE 98 (11) (2010)
 1903\-1917.
 
 \bibitem{27} K. Nair, J. Kulkarni, M. Warde, Z. Dave, V. Rawalgaonkar, G. Gore,
J. Joshi, Optimizing power consumption in iot based wireless sensor networks using bluetooth low energy, in: Green Computing and Internet of
Things (ICGCIoT), 2015 International Conference on, IEEE, 2015, pp.
 589\-593.
 
 \bibitem{28} G. Huang, J. He, Z. Ding, Wireless video-based sensor networks for surveillance of residential districts, in: Asia-Pacific Web Conference, Springer,
2008, pp. 154\-165.

 \bibitem{29} L.-m. Ang, K. P. Seng, L. W. Chew, L. S. Yeong, W. C. Chia, Wireless
 multimedia sensor networks on reconfigurable hardware (2013).
 \bibitem{30} Y. Zhou, W. Xiang, G. Wang, Frame loss concealment for multiview
video transmission over wireless multimedia sensor networks, IEEE Sensors Journal 15 (3) (2015) 1892\-1901.

 \bibitem{31} H. Shen, G. Bai, Routing in wireless multimedia sensor networks: A survey
 and challenges ahead, Journal of Network and Computer Applications 71
(2016) 30\-49.

 \bibitem{32} R. T. Collins, A. J. Lipton, H. Fujiyoshi, T. Kanade, Algorithms for cooperative multisensor surveillance, Proceedings of the IEEE 89 (10) (2001)
1456\-1477.

  \bibitem{33} H. Aghajan, A. Cavallaro, Multi-camera networks: principles and applications, Academic press, 2009.
 
 \bibitem{34} M. Valera, S. A. Velastin, Intelligent distributed surveillance systems: a review, IEE Proceedings-Vision, Image and Signal Processing 152 (2) (2005)
192\-204.

  \bibitem{35} C. Stauffer, K. Tieu, Automated multi-camera planar tracking correspondence modeling, in: Computer Vision and Pattern Recognition, 2003.
Proceedings. 2003 IEEE Computer Society Conference on, Vol. 1, IEEE,
2003, pp. 1\-1.

 \bibitem{36} G. Lu, B. Cheng, Q. Lin, Y. Wang, Quantitative indicator of homeostatic
 risk perception in car following, Safety science 50 (9) (2012) 1898\-1905.
 
 \bibitem{37} A. V. Kurilkin, O. O. Vyatkina, S. A. Mityagin, S. V. Ivanov, Evaluation
of urban mobility using surveillance cameras, Procedia Computer Science
66 (2015) 364\-371.

 \bibitem{38} F. Yin, D. Makris, S. A. Velastin, T. Ellis, Calibration and object corre-
 spondence in camera networks with widely separated overlapping views,
IET Computer Vision 9 (3) (2014) 354\-367.

 \bibitem{39} J. Sochor, R. Jur´anek, A. Herout, Traffic surveillance camera calibration
by 3d model bounding box alignment for accurate vehicle speed measurement, Computer Vision and Image Understanding 161 (2017) 87\-98.
 
 \bibitem{40} R. Xia, M. Hu, J. Zhao, S. Chen, Y. Chen, S. Fu, Global calibration of
non-overlapping cameras: State of the art, Optik-International Journal
for Light and Electron Optics.

 \bibitem{41} P. L´ebraly13, O. Ait-Aider13, E. Royer23, M. Dhome13, Calibration of
non-overlapping cameras-application to vision-based robotics, -.

  \bibitem{42} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker based
simple non-overlapping camera calibration, in: Image Processing (ICIP),
2016 IEEE International Conference on, IEEE, 2016, pp. 1180\-1184.

 \bibitem{43} S. Esquivel, F. Woelk, R. Koch, Calibration of a multi-camera rig
from non-overlapping views, in: Joint Pattern Recognition Symposium,
 Springer, 2007, pp. 82\-91.
 
 \bibitem{44} L. Heng, B. Li, M. Pollefeys, Camodocal: Automatic intrinsic and extrinsic calibration of a rig with multiple generic cameras and odometry,
in: Intelligent Robots and Systems (IROS), 2013 IEEE/RSJ International
Conference on, IEEE, 2013, pp. 1793\-1800.

  \bibitem{45} E. Ataer-Cansizoglu, Y. Taguchi, S. Ramalingam, Y. Miki, Calibration
of non-overlapping cameras using an external slam system, in: 3D Vision
(3DV), 2014 2nd International Conference on, Vol. 1, IEEE, 2014, pp.
509\-516.

 \bibitem{46} C. Forster, M. Pizzoli, D. Scaramuzza, Svo: Fast semi-direct monocu-
 lar visual odometry, in: Robotics and Automation (ICRA), 2014 IEEE
International Conference on, IEEE, 2014, pp. 15\-22.

 \bibitem{47} R. A. Newcombe, S. J. Lovegrove, A. J. Davison, Dtam: Dense tracking and mapping in real-time, in: Computer Vision (ICCV), 2011 IEEE
International Conference on, IEEE, 2011, pp. 2320\-2327.

  \bibitem{48} G. Carrera, A. Angeli, A. J. Davison, Slam-based automatic extrinsic
calibration of a multi-camera rig, in: Robotics and Automation (ICRA),
2011 IEEE International Conference on, IEEE, 2011, pp. 2652\-2659.

47 \bibitem{49} A. Agrawal, Extrinsic camera calibration without a direct view using
spherical mirror, in: Computer Vision (ICCV), 2013 IEEE International
 Conference on, IEEE, 2013, pp. 2368\-2375.
 
 \bibitem{50} R. K. Kumar, A. Ilie, J.-M. Frahm, M. Pollefeys, Simple calibration of
non-overlapping cameras with a mirror, in: Computer Vision and Pattern
Recognition, 2008. CVPR 2008. IEEE Conference on, IEEE, 2008, pp.
1\-7.

 \bibitem{51} K. Takahashi, S. Nobuhara, T. Matsuyama, A new mirror-based extrinsic
camera calibration using an orthogonality constraint, in: Computer Vision
and Pattern Recognition (CVPR), 2012 IEEE Conference on, IEEE, 2012,
pp. 1051\-1058.

 \bibitem{52} N. Anjum, M. Taj, A. Cavallaro, Relative position estimation of non-
 overlapping cameras, in: Acoustics, Speech and Signal Processing, 2007.
ICASSP 2007. IEEE International Conference on, Vol. 2, IEEE, 2007, pp.
II\-281.

 \bibitem{53} B. Lamprecht, S. Rass, S. Fuchs, K. Kyamakya, Extrinsic camera calibration for an on-board two-camera system without overlapping field of
 view, in: Intelligent Transportation Systems Conference, 2007. ITSC 2007.
IEEE, IEEE, 2007, pp. 265\-270.

 \bibitem{54} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker based
simple non-overlapping camera calibration, in: Image Processing (ICIP),
2016 IEEE International Conference on, IEEE, 2016, pp. 1180\-1184.

 \bibitem{55} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker-based
non-overlapping camera calibration methods with additional support camera views, Image and Vision Computing 70 (2018) 46\-54.

 \bibitem{56} P. F. Alcantarilla, C. Beall, F. Dellaert, Large-scale dense 3d reconstruction from stereo imagery, in: Computational Perception and Robotics,
 Georgia Institute of Technology, 2013, pp. 1\-6.
 
 \bibitem{57} I. Kitahara, H. Saito, S. Akimichi, T. Ono, Y. Ohta, T. Kanade, Largescale virtualized reality, Computer Vision and Pattern Recognition, Technical Sketches.

 \bibitem{58} R. Lu, Y. Li, A global calibration method for large-scale multi-sensor
 visual measurement systems, Sensors and Actuators A: Physical 116 (3)
(2004) 384\-393.

 \bibitem{59} C. Jianhui, R. Shunan, W. Guolei, Y. Xiangdong, C. Ken, Calibration
and compensation to large-scale multi-robot motion platform using laser
tracker, in: Cyber Technology in Automation, Control, and Intelligent
 Systems (CYBER), 2015 IEEE International Conference on, IEEE, 2015,
pp. 163\-168.

 \bibitem{60} A. Ortega, B. Dias, E. Teniente, A. Bernardino, J. Gaspar, J. AndradeCetto, Calibrating an outdoor distributed camera network using laser
range finder data, in: Intelligent Robots and Systems, 2009. IROS 2009.
 IEEE/RSJ International Conference on, IEEE, 2009, pp. 303\-308.
 
 \bibitem{61} G. Chen, Y. Guo, H. Wang, D. Ye, Y. Gu, Stereo vision sensor calibration based on random spatial points given by cmm, Optik-International
Journal for Light and Electron Optics 123 (8) (2012) 731\-734.

 \bibitem{62} H. Bingwei, W. Gongjian, Z. Xing, L. Deren, Accurate geometric camera
 calibration technique using multi-views of a non-metric planar grid, Optics
and Lasers in Engineering 51 (4) (2013) 432\-439.

 \bibitem{63} T. Strauß, J. Ziegler, J. Beck, Calibrating multiple cameras with non overlapping views using coded checkerboard targets, in: Intelligent Transportation Systems (ITSC), 2014 IEEE 17th International Conference on,
 IEEE, 2014, pp. 2623\-2628.
 
 \bibitem{64} D. Zhan, L. Yu, J. Xiao, T. Chen, Multi-camera and structured-light vision system (msvs) for dynamic high-accuracy 3d measurements of railway
tunnels, Sensors 15 (4) (2015) 8664\-8684.

\bibitem{65} J. Sun, H. He, D. Zeng, Global calibration of multiple cameras based on
 sphere targets, Sensors 16 (1) (2016) 77.
 
 \bibitem{66} X. Wu, S. Wu, Z. Xing, X. Jia, A global calibration method for widely
distributed cameras based on vanishing features, Sensors 16 (6) (2016)
838.

 \bibitem{67} F. Vasconcelos, J. P. Barreto, E. Boyer, Automatic camera calibration
 using multiple sets of pairwise correspondences, IEEE transactions on
pattern analysis and machine intelligence 40 (4) (2018) 791\-803.

 \bibitem{68} Q. Wang, Q. Zhang, F. Rovira-Mas, Auto-calibration method to determine
camera pose for stereovision-based off-road vehicle navigation, Environmental Control in Biology 48 (2) (2010) 59\-72.

  \bibitem{69} R. Pflugfelder, H. Bischof, Localization and trajectory reconstruction in
surveillance cameras with nonoverlapping views, IEEE Transactions on
Pattern Analysis and Machine Intelligence 32 (4) (2010) 709\-721.

 \bibitem{70} Q. Wang, Y. Liu, Y. Shen, An accurate extrinsic camera self-calibration
method in non-overlapping camera sensor networks, in: Instrumentation
 and Measurement Technology Conference (I2MTC), 2011 IEEE, IEEE,
2011, pp. 1\-6.

 \bibitem{71} Q. Wang, Y. Liu, A tractable mechanism for external calibration in nonoverlapping camera network, in: Communications and Networking in
China (CHINACOM), 2011 6th International ICST Conference on, IEEE,
 2011, pp. 893\-898.
 
 \bibitem{72} F. Pagel, Extrinsic self-calibration of multiple cameras with nonoverlapping views in vehicles, in: Video Surveillance and Transportation
Imaging Applications 2014, Vol. 9026, International Society for Optics
and Photonics, 2014, p. 902606.

 \bibitem{73} H. Huang, N. Li, H. Guo, Y.-L. Chen, X. Wu, Calibration of nonoverlapping cameras based on a mobile robot, in: Information Science
50and Technology (ICIST), 2015 5th International Conference on, IEEE,
2015, pp. 328\-333.
 \bibitem{74} Q. Liu, J. Sun, Z. Liu, G. Zhang, Global calibration method of multi-
 sensor vision system using skew laser lines, Chinese Journal of Mechanical
Engineering 25 (2) (2012) 405\-410.

 \bibitem{75} Z. Liu, X. Wei, G. Zhang, External parameter calibration of widely distributed vision sensors with non-overlapping fields of view, Optics and
Lasers in Engineering 51 (6) (2013) 643\-650.

 \bibitem{76} W. Zou, S. Li, Calibration of nonoverlapping in-vehicle cameras with laser
pointers, IEEE Transactions on Intelligent Transportation Systems 16 (3)
(2015) 1348\-1359.

 \bibitem{77} W. Zou, Calibrating non-overlapping cameras with a laser ray, Ph.D. thesis, Tottori University (2015).

 \bibitem{78} M. Nischt, R. Swaminathan, Self-calibration of asynchronized camera networks, in: Computer Vision Workshops (ICCV Workshops), 2009 IEEE
12th International Conference on, IEEE, 2009, pp. 2164\-2171.

 \bibitem{79} S. Dong, X. Shao, X. Kang, F. Yang, X. He, Extrinsic calibration of a
non-overlapping camera network based on close-range photogrammetry,
 Applied optics 55 (23) (2016) 6363\-6370.

 \bibitem{80} H. Hu, J. Liang, Z.-Z. Tang, B.-Q. Shi, X. Guo, Global calibration
for multi-camera videogrammetric system with large-scale field-of-view,
Guangxue Jingmi Gongcheng(Optics and Precision Engineering) 20 (2)
(2012) 369\-378.


 \bibitem{81} T. Birdal, E. Bala, T. Eren, S. Ilic, Online inspection of 3d parts via a
locally overlapping camera network, in: Applications of Computer Vision
(WACV), 2016 IEEE Winter Conference on, IEEE, 2016, pp. 1\-10.

 \bibitem{82} D. J. Cook, J. C. Augusto, V. R. Jakkula, Ambient intelligence: Technologies, applications, and opportunities, Pervasive and Mobile Computing
 5 (4) (2009) 277\-298.

 \bibitem{83} T. E. McSween, Values-based safety process: Improving your safety culture with behavior-based safety, John Wiley \& Sons, 2003.

 \bibitem{84} C. Fuller, An assessment of the relationship between behaviour and injury
in the workplace: A case study in professional football, Safety science
 43 (4) (2005) 213\-224.

 \bibitem{85} N. J. Bahr, System safety engineering and risk assessment: a practical
approach, CRC Press, 2014.

 \bibitem{86} T. Kongsvik, J. Fenstad, C. Wendelborg, Between a rock and a hard place:
Accident and near-miss reporting on offshore service vessels, Safety science
 50 (9) (2012) 1839\-1846.

 \bibitem{87} H. Li, M. Lu, S.-C. Hsu, M. Gray, T. Huang, Proactive behavior-based
safety management for construction safety improvement, Safety science
75 (2015) 107\-117.

 \bibitem{88} A. M. Shariff, N. Norazahar, At-risk behaviour analysis and improvement
 study in an academic laboratory, Safety science 50 (1) (2012) 29-38.

 \bibitem{89} C. Qing-gui, L. Kai, L. Ye-jiao, S. Qi-hua, Z. Jian, Risk management and
workers safety behavior control in coal mine, Safety science 50 (4) (2012)
909\-913.
 \bibitem{90} A. Laureshyn, Application of automated video analysis to road user behaviour, 2010.

\item \relax [91} T. Lv, H.-y. Zhang, C.-h. Yan, Double mode surveillance system based
on remote audio/video signals acquisition, Applied Acoustics 129 (2018)
316\-321.

 \bibitem{92} Y. Qu, T. Wang, Z. Zhu, Remote audio/video acquisition for human signa-
 ture detection, in: Computer Vision and Pattern Recognition Workshops,
2009. CVPR Workshops 2009. IEEE Computer Society Conference on,
IEEE, 2009, pp. 66\-71.

 \bibitem{93} H.-y. Zhang, T. Lv, C. Yan, The novel role of arctangent phase algorithm
and voice enhancement techniques in laser hearing, Applied Acoustics 126
 (2017) 136\-142.

 \bibitem{94} M. Kyriakidis, R. Hirsch, A. Majumdar, Metro railway safety: An analysis
of accident precursors, Safety science 50 (7) (2012) 1535\-1548.

 \bibitem{95} S. Andriulo, M. G. Gnoni, Measuring the effectiveness of a near-miss management system: An application in an automotive firm supplier, Reliability Engineering \& System Safety 132 (2014) 154\-162.

 \bibitem{96} S. C. Lubobya, M. E. Dlodlo, G. De Jager, A. Zulu, Throughput characteristics of wimax video surveillance systems, Procedia Computer Science
45 (2015) 571\-580.

 \bibitem{97} M.-J. Yang, J. Y. Tham, D. Wu, K. H. Goh, Cost effective ip camera
 for video surveillance, in: Industrial Electronics and Applications, 2009.
ICIEA 2009. 4th IEEE Conference on, IEEE, 2009, pp. 2432\-2435.

 \bibitem{98} B. Gumaidah, H. Soliman, Wimax network performance improvement
through the optimal use of available bandwidth by adaptive selective voice
coding, International Journal of Modern Engineering Sciences 2 (1) (2013)
1\-16.

 \bibitem{99} J. Changjiang, W. Jin, L. Mingfu, L. Zhichuan, A design and implementation of mobile video surveillance terminal base on arm, Procedia Computer
Science 107 (2017) 498\-502.

 \bibitem{100} N. Chen, Y. Chen, Y. You, H. Ling, P. Liang, R. Zimmermann, Dynamic
urban surveillance video stream processing using fog computing, in: Mul-
53timedia Big Data (BigMM), 2016 IEEE Second International Conference
on, IEEE, 2016, pp. 105\-112.

 \bibitem{101} D. A. Rodr´ıguez-Silva, L. Adkinson-Orellana, F. Gonz’lez-Castano,
I. Armino-Franco, D. Gonz’lez-Martinez, Video surveillance based on
 cloud storage, in: Cloud Computing (CLOUD), 2012 IEEE 5th International Conference on, IEEE, 2012, pp. 991\-992.

 \bibitem{102} N. Chen, Y. Chen, S. Song, C.-T. Huang, X. Ye, Smart urban surveillance
using fog computing, in: Edge Computing (SEC), IEEE/ACM Symposium on, IEEE, 2016, pp. 95\-96.

 \bibitem{103} H. Sun, X. Liang, W. Shi, Vu: video usefulness and its application in largescale video surveillance systems: an early experience, in: Proceedings of
the Workshop on Smart Internet of Things, ACM, 2017, p. 6.

 \bibitem{104} Q. Zhang, Z. Yu, W. Shi, H. Zhong, Demo abstract: Evaps: Edge video
analysis for public safety, in: Edge Computing (SEC), IEEE/ACM Symposium on, IEEE, 2016, pp. 121\-122.

 \bibitem{105} R. Du, S. Bista, A. Varshney, Video fields: fusing multiple surveillance
videos into a dynamic virtual environment, in: Proceedings of the 21st
International Conference on Web3D Technology, ACM, 2016, pp. 165\-172.

 \bibitem{106} S. Singh, C. Shekhar, A. Vohra, Fpga-based real-time motion detection
for automated video surveillance systems, Electronics 5 (1) (2016) 10.

 \bibitem{107} Y. Li, R. Xia, Q. Huang, W. Xie, X. Li, Survey of spatio-temporal interest
point detection algorithms in video, IEEE Access 5 (2017) 10323\-10331.

 \bibitem{108} B. Tian, B. T. Morris, M. Tang, Y. Liu, Y. Yao, C. Gou, D. Shen, S. Tang,
 Hierarchical and networked vehicle surveillance in its: A survey, IEEE
Transactions on Intelligent Transportation Systems 18 (1) (2017) 25-48.

 \bibitem{109} T. Bouwmans, A. Sobral, S. Javed, S. K. Jung, E.-H. Zahzah, Decomposition into low-rank plus additive matrices for background/foreground separation: A review for a comparative evaluation with a large-scale dataset,
Computer Science Review 23 (2017) 1-71.

 \bibitem{110} O. Elharrouss, A. Abbad, D. Moujahid, H. Tairi, Moving object detection
zone using a block-based background model, IET Computer Vision 12 (1)
(2017) 86-94.

 \bibitem{111} O. Elharrouss, D. Moujahid, S. Elkah, H. Tairi, Moving object detection
 using a background modeling based on entropy theory and quad-tree decomposition, Journal of Electronic Imaging 25 (6) (2016) 061615.

 \bibitem{112} E. Cerme~no, A. P´erez, J. A. Sig¨uenza, Intelligent video surveillance beyond robust background modeling, Expert Systems with Applications 91
(2018) 138-149.

 \bibitem{113} F.-C. Cheng, S.-C. Huang, S.-J. Ruan, Illumination-sensitive background
modeling approach for accurate moving object detection, IEEE Transactions on broadcasting 57 (4) (2011) 794-801.

 \bibitem{114} Y. Wang, Q. Lu, D. Wang, W. Liu, Compressive background modeling for
foreground extraction, Journal of Electrical and Computer Engineering
2015 (2015) 13.

 \bibitem{115} B.-H. Chen, S.-C. Huang, J.-Y. Yen, Counter-propagation artificial neural
network-based motion detection algorithm for static-camera surveillance
scenarios, Neurocomputing 273 (2018) 481-493.

 \bibitem{116} W. Bouachir, R. Noumeir, Automated video surveillance for preventing
suicide attempts.

 \bibitem{117} W. Bouachir, R. Gouiaa, B. Li, R. Noumeir, Intelligent video surveillance
for real-time detection of suicide attempts, Pattern Recognition Letters
110 (2018) 1-7.

 \bibitem{118} R. Kachach, J. M. Ca~nas, Hybrid three-dimensional and support vector
machine approach for automatic vehicle tracking and classification using
a single camera, Journal of Electronic Imaging 25 (3) (2016) 033021.

 \bibitem{119} Y. Dedeo˘glu, B. U. T¨oreyin, U. Gudukbay, A. E. C¸ etin, Silhouette-based
method for object classification and human action recognition in video,
in: European Conference on Computer Vision, Springer, 2006, pp. 64-77.

 \bibitem{120} F. Wu, X.-Y. Jing, X. You, D. Yue, R. Hu, J.-Y. Yang, Multi-view lowrank dictionary learning for image classification, Pattern Recognition 50
(2016) 143-154.


 \bibitem{121} M. Imani, H. Ghassemian, Edge-preserving-based collaborative representation for spectral-spatial classification, International Journal of Remote
 Sensing 38 (20) (2017) 5524-5545.

 \bibitem{122} Y. Gurwicz, R. Yehezkel, B. Lachover, Multiclass object classification for
real-time video surveillance systems, Pattern Recognition Letters 32 (6)
(2011) 805-815.

 \bibitem{123} N. Najva, K. E. Bijoy, Sift and tensor based object detection and classification in videos using deep neural networks, Procedia Computer Science
93 (2016) 351-358.

 \bibitem{124} M. U. Yaseen, A. Anjum, O. Rana, R. Hill, Cloud-based scalable object
detection and classification in video streams, Future Generation Computer
Systems 80 (2018) 286-298.

 \bibitem{125} I. Elafi, M. Jedra, N. Zahid, Unsupervised detection and tracking of moving objects for video surveillance applications, Pattern Recognition Letters
84 (2016) 70-77.

 \bibitem{126} X. Li, W. Hu, C. Shen, Z. Zhang, A. Dick, A. V. D. Hengel, A survey of
appearance models in visual object tracking, ACM transactions on Intelligent Systems and Technology (TIST) 4 (4) (2013) 58.

 \bibitem{127} D. Moujahid, O. Elharrouss, H. Tairi, Visual object tracking via the local
soft cosine similarity, Pattern Recognition Letters 110 (2018) 79-85.

 \bibitem{128} D. Moujahid, O. Elharrouss, H. Tairi, Visual moving object tracking via
sparse representation based trackers: A comparative study, in: Complex
Systems (WCCS), 2015 Third World Conference on, IEEE, 2015, pp. 1-6.

 \bibitem{129} A. W. Smeulders, D. M. Chu, R. Cucchiara, S. Calderara, A. Dehghan,
M. Shah, Visual tracking: An experimental survey, IEEE transactions on
pattern analysis and machine intelligence 36 (7) (2014) 1442-1468.

 \bibitem{130} Z. Kalal, K. Mikolajczyk, J. Matas, Tracking-learning-detection, IEEE
 transactions on pattern analysis and machine intelligence 34 (7) (2012)
1409-1422.

 \bibitem{131} B. Zhuang, H. Lu, Z. Xiao, D. Wang, Visual tracking via discriminative
sparse similarity map, IEEE Transactions on Image Processing 23 (4)
(2014) 1872-1881.

 \bibitem{132} X. Cheng, N. Li, T. Zhou, L. Zhou, Z. Wu, Object tracking via collaborative multi-task learning and appearance model updating, Applied Soft
Computing 31 (2015) 81-90.

 \bibitem{133} W. Zhong, H. Lu, M.-H. Yang, Robust object tracking via sparse collaborative appearance model, IEEE Transactions on Image Processing 23 (5)
 (2014) 2356-2368.

 \bibitem{134} S. Murthy, B. Sujatha, Multi-level optimization in encoding to balance
video compression and retention of 8k resolution, Perspectives in Science
8 (2016) 338-344.

 \bibitem{135} N. Patil, S. Ambatkar, S. Kakde, Iot based smart surveillance security
system using raspberry pi, in: Communication and Signal Processing
(ICCSP), 2017 International Conference on, IEEE, 2017, pp. 0344-0348.

 \bibitem{136} D. Minoli, K. Sohraby, B. Occhiogrosso, Iot considerations, requirements, and architectures for smart buildingsenergy optimization and nextgeneration building management systems, IEEE Internet of Things Journal 4 (1) (2017) 269-283.

 \bibitem{137} A. Khan, B. Rinner, A. Cavallaro, Cooperative robots to observe moving
targets, IEEE transactions on cybernetics.

 \bibitem{138} S. Zhu, Z. Xu, Spatiotemporal visual saliency guided perceptual high efficiency video coding with neural network, Neurocomputing 275 (2018)
 511-522.

 \bibitem{139} J. Galan-Hernandez, V. Alarcon-Aquino, O. Starostenko, J. RamirezCortes, P. Gomez-Gil, Wavelet-based frame video coding algorithms using fovea and speck, Engineering Applications of Artificial Intelligence 69
(2018) 127-136.

 \bibitem{140} N. Chen, Y. Chen, X. Ye, H. Ling, S. Song, C.-T. Huang, Smart city
surveillance in fog computing, in: Advances in Mobile Cloud Computing
and Big Data in the 5G Era, Springer, 2017, pp. 203-226.

 \bibitem{141} A. J. Neto, Z. Zhao, J. J. Rodrigues, H. B. Camboim, T. Braun, Fogbased crime-assistance in smart iot transportation system, IEEE Access
6 (2018) 11101-11111.

 \bibitem{142} S. Chen, T. Zhang, W. Shi, Fog computing, IEEE Internet Computing
21 (2) (2017) 4-6.

 \bibitem{143} X. Yue, Y. Liu, J. Wang, H. Song, H. Cao, Software defined radio and
wireless acoustic networking for amateur drone surveillance, IEEE Com-
 munications Magazine 56 (4) (2018) 90-97.

 \bibitem{144} S. Baidya, M. Levorato, Content-aware cognitive interference control for
urban iot systems, IEEE Transactions on Cognitive Communications and
Networking.


\end{thebibliography}


==> references.tex <==
\begin{thebibliography}{00}

 \bibitem{1}     F. Porikli, F. Br´emond, S. L. Dockstader, J. Ferryman, A. Hoogs, B. C.
Lovell, S. Pankanti, B. Rinner, P. Tu, P. L. Venetianer, Video surveillance:
 past, present, and now the future [dsp forum}, IEEE Signal Processing
Magazine 30 (3) (2013) 190\-198.

 \bibitem{2} D. Cumming, S. Johan, Cameras tracking shoppers: the economics of
retail video surveillance, Eurasian Business Review 5 (2) (2015) 235\-257.

 \bibitem{3} Y. Tang, B. Ma, H. Yan, Intelligent video surveillance system for elderly
 people living alone based on odvs, Advances in Internet of Things 3 (02)
(2013)

 \bibitem{4} J. M. Such, A. Espinosa, A. Garc´ıa-Fornes, A survey of privacy in multiagent systems, The Knowledge Engineering Review 29 (3) (2014) 314\-344.

 \bibitem{5} M. Cristani, R. Raghavendra, A. Del Bue, V. Murino, Human behav-
 ior analysis in video surveillance: A social signal processing perspective,
Neurocomputing 100 (2013) 86\-97.
 \bibitem{6} A. G. Bole, W. O. Dineley, A. Wall, Radar and ARPA manual, Elsevier
Butterworth Heinemann, 2005.

 \bibitem{7} J. Lubczonek, A. Stateczny, Aspects of spatial planning of radar sensor
 network for inland waterways surveillance, in: Radar Conference, 2009.
EuRAD 2009. European, IEEE, 2009, pp. 501\-504.
 \bibitem{8} A. Borkowski, Filtering of aerial laser scanning data by active surface
model, Annals of Geomatics 2006 3 (4).

 \bibitem{9} R. T. Collins, A. J. Lipton, T. Kanade, Introduction to the special section
 on video surveillance, IEEE Transactions on pattern analysis and machine
intelligence 22 (8) (2000) 745\-746.

 \bibitem{10} Z. Xu, Y. Liu, L. Mei, C. Hu, L. Chen, Semantic based representing
and organizing surveillance big data using video structural description
technology, Journal of Systems and Software 102 (2015) 217\-225.

  \item \relax  [11} Z. Xu, C. Hu, L. Mei, Video structured description technology based
intelligence analysis of surveillance videos for public security applications,
Multimedia Tools and Applications 75 (19) (2016) 12155\-12172.

 \bibitem{12} O. El Harrouss, D. Moujahid, H. Tairi, Motion detection based on the
combining of the background subtraction and spatial color information,
 in: Intelligent Systems and Computer Vision (ISCV), 2015, IEEE, 2015,
pp. 1\-4.

 \bibitem{13} S. Khokhar, I. Saleemi, M. Shah, Multi-agent event recognition by preservation of spatiotemporal relationships between probabilistic models, Image and Vision Computing 31 (9) (2013) 603\-615.

  \item \relax  [14} H. Wang, A. Kl¨aser, C. Schmid, C.-L. Liu, Dense trajectories and motion boundary descriptors for action recognition, International journal of
computer vision 103 (1) (2013) 60\-79.

 \bibitem{15} H. Wang, C. Yuan, W. Hu, H. Ling, W. Yang, C. Sun, Action recognition using nonnegative action component representation and sparse basis
 selection, IEEE transactions on image processing 23 (2) (2014) 570\-581.
 
 \bibitem{16} T. E. Boult, R. J. Micheals, X. Gao, M. Eckmann, Into the woods: Visual surveillance of noncooperative and camouflaged targets in complex
outdoor settings, Proceedings of the IEEE 89 (10) (2001) 1382\-1402.

 \bibitem{17} C. P. Diehl, Toward efficient collaborative classification for distributed
 video surveillance, Ph.D. thesis, Citeseer (2000).
 
 \item \relax [18} D. M. Gavrila, The visual analysis of human movement: A survey, Computer vision and image understanding 73 (1) (1999) 82\-98.

 \bibitem{19} J. Templer, J. Archea, H. H. Chen, Study of factors associated with risk
of work-related stairway falls, Journal of Safety Research 16 (4) (1985)
 183\-196.
 \bibitem{20} T. Cav´en, J. Saari, Videotape-based interviews in safety analysis, Journal
of Occupational Accidents 4 (2-4) (1982) 341\-345.

 \bibitem{21} P. Cocca, F. Marciano, D. Rossi, Assessment of biomechanical risk at
work: practical approaches and tools, Acta of bioengineering and biome-
 chanics 10 (3) (2008) 21\-27.
 
 \bibitem{22} G. David, Ergonomic methods for assessing exposure to risk factors
for work-related musculoskeletal disorders, Occupational medicine 55 (3)
(2005) 190\-99.

 \bibitem{23} G. L. Foresti, P. Mahonen, C. S. Regazzoni, Multimedia video-based
 surveillance systems: Requirements, Issues and Solutions, Vol. 573,
Springer Science \& Business Media, 2012.
 \bibitem{24} P. Natarajan, P. K. Atrey, M. Kankanhalli, Multi-camera coordination
and control in surveillance systems: A survey, ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM) 11 (4)
 (2015) 57.
 \bibitem{25} D. Stepanov, I. Tishchenko, The concept of video surveillance system
based on the principles of stereo vision., in: FRUCT, 2016, pp. 328\-334.

 \bibitem{26} P. Corke, T. Wark, R. Jurdak, W. Hu, P. Valencia, D. Moore, Environmental wireless sensor networks, Proceedings of the IEEE 98 (11) (2010)
 1903\-1917.
 
 \bibitem{27} K. Nair, J. Kulkarni, M. Warde, Z. Dave, V. Rawalgaonkar, G. Gore,
J. Joshi, Optimizing power consumption in iot based wireless sensor networks using bluetooth low energy, in: Green Computing and Internet of
Things (ICGCIoT), 2015 International Conference on, IEEE, 2015, pp.
 589\-593.
 
 \bibitem{28} G. Huang, J. He, Z. Ding, Wireless video-based sensor networks for surveillance of residential districts, in: Asia-Pacific Web Conference, Springer,
2008, pp. 154\-165.

 \bibitem{29} L.-m. Ang, K. P. Seng, L. W. Chew, L. S. Yeong, W. C. Chia, Wireless
 multimedia sensor networks on reconfigurable hardware (2013).
 \bibitem{30} Y. Zhou, W. Xiang, G. Wang, Frame loss concealment for multiview
video transmission over wireless multimedia sensor networks, IEEE Sensors Journal 15 (3) (2015) 1892\-1901.

 \bibitem{31} H. Shen, G. Bai, Routing in wireless multimedia sensor networks: A survey
 and challenges ahead, Journal of Network and Computer Applications 71
(2016) 30\-49.

 \bibitem{32} R. T. Collins, A. J. Lipton, H. Fujiyoshi, T. Kanade, Algorithms for cooperative multisensor surveillance, Proceedings of the IEEE 89 (10) (2001)
1456\-1477.

  \bibitem{33} H. Aghajan, A. Cavallaro, Multi-camera networks: principles and applications, Academic press, 2009.
 
 \bibitem{34} M. Valera, S. A. Velastin, Intelligent distributed surveillance systems: a review, IEE Proceedings-Vision, Image and Signal Processing 152 (2) (2005)
192\-204.

  \bibitem{35} C. Stauffer, K. Tieu, Automated multi-camera planar tracking correspondence modeling, in: Computer Vision and Pattern Recognition, 2003.
Proceedings. 2003 IEEE Computer Society Conference on, Vol. 1, IEEE,
2003, pp. 1\-1.

 \bibitem{36} G. Lu, B. Cheng, Q. Lin, Y. Wang, Quantitative indicator of homeostatic
 risk perception in car following, Safety science 50 (9) (2012) 1898\-1905.
 
 \bibitem{37} A. V. Kurilkin, O. O. Vyatkina, S. A. Mityagin, S. V. Ivanov, Evaluation
of urban mobility using surveillance cameras, Procedia Computer Science
66 (2015) 364\-371.

 \bibitem{38} F. Yin, D. Makris, S. A. Velastin, T. Ellis, Calibration and object corre-
 spondence in camera networks with widely separated overlapping views,
IET Computer Vision 9 (3) (2014) 354\-367.

 \bibitem{39} J. Sochor, R. Jur´anek, A. Herout, Traffic surveillance camera calibration
by 3d model bounding box alignment for accurate vehicle speed measurement, Computer Vision and Image Understanding 161 (2017) 87\-98.
 
 \bibitem{40} R. Xia, M. Hu, J. Zhao, S. Chen, Y. Chen, S. Fu, Global calibration of
non-overlapping cameras: State of the art, Optik-International Journal
for Light and Electron Optics.

 \bibitem{41} P. L´ebraly13, O. Ait-Aider13, E. Royer23, M. Dhome13, Calibration of
non-overlapping cameras-application to vision-based robotics, -.

  \bibitem{42} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker based
simple non-overlapping camera calibration, in: Image Processing (ICIP),
2016 IEEE International Conference on, IEEE, 2016, pp. 1180\-1184.

 \bibitem{43} S. Esquivel, F. Woelk, R. Koch, Calibration of a multi-camera rig
from non-overlapping views, in: Joint Pattern Recognition Symposium,
 Springer, 2007, pp. 82\-91.
 
 \bibitem{44} L. Heng, B. Li, M. Pollefeys, Camodocal: Automatic intrinsic and extrinsic calibration of a rig with multiple generic cameras and odometry,
in: Intelligent Robots and Systems (IROS), 2013 IEEE/RSJ International
Conference on, IEEE, 2013, pp. 1793\-1800.

  \bibitem{45} E. Ataer-Cansizoglu, Y. Taguchi, S. Ramalingam, Y. Miki, Calibration
of non-overlapping cameras using an external slam system, in: 3D Vision
(3DV), 2014 2nd International Conference on, Vol. 1, IEEE, 2014, pp.
509\-516.

 \bibitem{46} C. Forster, M. Pizzoli, D. Scaramuzza, Svo: Fast semi-direct monocu-
 lar visual odometry, in: Robotics and Automation (ICRA), 2014 IEEE
International Conference on, IEEE, 2014, pp. 15\-22.

 \bibitem{47} R. A. Newcombe, S. J. Lovegrove, A. J. Davison, Dtam: Dense tracking and mapping in real-time, in: Computer Vision (ICCV), 2011 IEEE
International Conference on, IEEE, 2011, pp. 2320\-2327.

  \bibitem{48} G. Carrera, A. Angeli, A. J. Davison, Slam-based automatic extrinsic
calibration of a multi-camera rig, in: Robotics and Automation (ICRA),
2011 IEEE International Conference on, IEEE, 2011, pp. 2652\-2659.

47 \bibitem{49} A. Agrawal, Extrinsic camera calibration without a direct view using
spherical mirror, in: Computer Vision (ICCV), 2013 IEEE International
 Conference on, IEEE, 2013, pp. 2368\-2375.
 
 \bibitem{50} R. K. Kumar, A. Ilie, J.-M. Frahm, M. Pollefeys, Simple calibration of
non-overlapping cameras with a mirror, in: Computer Vision and Pattern
Recognition, 2008. CVPR 2008. IEEE Conference on, IEEE, 2008, pp.
1\-7.

 \bibitem{51} K. Takahashi, S. Nobuhara, T. Matsuyama, A new mirror-based extrinsic
camera calibration using an orthogonality constraint, in: Computer Vision
and Pattern Recognition (CVPR), 2012 IEEE Conference on, IEEE, 2012,
pp. 1051\-1058.

 \bibitem{52} N. Anjum, M. Taj, A. Cavallaro, Relative position estimation of non-
 overlapping cameras, in: Acoustics, Speech and Signal Processing, 2007.
ICASSP 2007. IEEE International Conference on, Vol. 2, IEEE, 2007, pp.
II\-281.

 \bibitem{53} B. Lamprecht, S. Rass, S. Fuchs, K. Kyamakya, Extrinsic camera calibration for an on-board two-camera system without overlapping field of
 view, in: Intelligent Transportation Systems Conference, 2007. ITSC 2007.
IEEE, IEEE, 2007, pp. 265\-270.

 \bibitem{54} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker based
simple non-overlapping camera calibration, in: Image Processing (ICIP),
2016 IEEE International Conference on, IEEE, 2016, pp. 1180\-1184.

 \bibitem{55} F. Zhao, T. Tamaki, T. Kurita, B. Raytchev, K. Kaneda, Marker-based
non-overlapping camera calibration methods with additional support camera views, Image and Vision Computing 70 (2018) 46\-54.

 \bibitem{56} P. F. Alcantarilla, C. Beall, F. Dellaert, Large-scale dense 3d reconstruction from stereo imagery, in: Computational Perception and Robotics,
 Georgia Institute of Technology, 2013, pp. 1\-6.
 
 \bibitem{57} I. Kitahara, H. Saito, S. Akimichi, T. Ono, Y. Ohta, T. Kanade, Largescale virtualized reality, Computer Vision and Pattern Recognition, Technical Sketches.

 \bibitem{58} R. Lu, Y. Li, A global calibration method for large-scale multi-sensor
 visual measurement systems, Sensors and Actuators A: Physical 116 (3)
(2004) 384\-393.

 \bibitem{59} C. Jianhui, R. Shunan, W. Guolei, Y. Xiangdong, C. Ken, Calibration
and compensation to large-scale multi-robot motion platform using laser
tracker, in: Cyber Technology in Automation, Control, and Intelligent
 Systems (CYBER), 2015 IEEE International Conference on, IEEE, 2015,
pp. 163\-168.

 \bibitem{60} A. Ortega, B. Dias, E. Teniente, A. Bernardino, J. Gaspar, J. AndradeCetto, Calibrating an outdoor distributed camera network using laser
range finder data, in: Intelligent Robots and Systems, 2009. IROS 2009.
 IEEE/RSJ International Conference on, IEEE, 2009, pp. 303\-308.
 
 \bibitem{61} G. Chen, Y. Guo, H. Wang, D. Ye, Y. Gu, Stereo vision sensor calibration based on random spatial points given by cmm, Optik-International
Journal for Light and Electron Optics 123 (8) (2012) 731\-734.

 \bibitem{62} H. Bingwei, W. Gongjian, Z. Xing, L. Deren, Accurate geometric camera
 calibration technique using multi-views of a non-metric planar grid, Optics
and Lasers in Engineering 51 (4) (2013) 432\-439.

 \bibitem{63} T. Strauß, J. Ziegler, J. Beck, Calibrating multiple cameras with non overlapping views using coded checkerboard targets, in: Intelligent Transportation Systems (ITSC), 2014 IEEE 17th International Conference on,
 IEEE, 2014, pp. 2623\-2628.
 
 \bibitem{64} D. Zhan, L. Yu, J. Xiao, T. Chen, Multi-camera and structured-light vision system (msvs) for dynamic high-accuracy 3d measurements of railway
tunnels, Sensors 15 (4) (2015) 8664\-8684.

\bibitem{65} J. Sun, H. He, D. Zeng, Global calibration of multiple cameras based on
 sphere targets, Sensors 16 (1) (2016) 77.
 
 \bibitem{66} X. Wu, S. Wu, Z. Xing, X. Jia, A global calibration method for widely
distributed cameras based on vanishing features, Sensors 16 (6) (2016)
838.

 \bibitem{67} F. Vasconcelos, J. P. Barreto, E. Boyer, Automatic camera calibration
 using multiple sets of pairwise correspondences, IEEE transactions on
pattern analysis and machine intelligence 40 (4) (2018) 791\-803.

 \bibitem{68} Q. Wang, Q. Zhang, F. Rovira-Mas, Auto-calibration method to determine
camera pose for stereovision-based off-road vehicle navigation, Environmental Control in Biology 48 (2) (2010) 59\-72.

  \bibitem{69} R. Pflugfelder, H. Bischof, Localization and trajectory reconstruction in
surveillance cameras with nonoverlapping views, IEEE Transactions on
Pattern Analysis and Machine Intelligence 32 (4) (2010) 709\-721.

 \bibitem{70} Q. Wang, Y. Liu, Y. Shen, An accurate extrinsic camera self-calibration
method in non-overlapping camera sensor networks, in: Instrumentation
 and Measurement Technology Conference (I2MTC), 2011 IEEE, IEEE,
2011, pp. 1\-6.

 \bibitem{71} Q. Wang, Y. Liu, A tractable mechanism for external calibration in nonoverlapping camera network, in: Communications and Networking in
China (CHINACOM), 2011 6th International ICST Conference on, IEEE,
 2011, pp. 893\-898.
 
 \bibitem{72} F. Pagel, Extrinsic self-calibration of multiple cameras with nonoverlapping views in vehicles, in: Video Surveillance and Transportation
Imaging Applications 2014, Vol. 9026, International Society for Optics
and Photonics, 2014, p. 902606.

 \bibitem{73} H. Huang, N. Li, H. Guo, Y.-L. Chen, X. Wu, Calibration of nonoverlapping cameras based on a mobile robot, in: Information Science
50and Technology (ICIST), 2015 5th International Conference on, IEEE,
2015, pp. 328\-333.
 \bibitem{74} Q. Liu, J. Sun, Z. Liu, G. Zhang, Global calibration method of multi-
 sensor vision system using skew laser lines, Chinese Journal of Mechanical
Engineering 25 (2) (2012) 405\-410.

 \bibitem{75} Z. Liu, X. Wei, G. Zhang, External parameter calibration of widely distributed vision sensors with non-overlapping fields of view, Optics and
Lasers in Engineering 51 (6) (2013) 643\-650.

 \bibitem{76} W. Zou, S. Li, Calibration of nonoverlapping in-vehicle cameras with laser
pointers, IEEE Transactions on Intelligent Transportation Systems 16 (3)
(2015) 1348\-1359.

 \bibitem{77} W. Zou, Calibrating non-overlapping cameras with a laser ray, Ph.D. thesis, Tottori University (2015).

 \bibitem{78} M. Nischt, R. Swaminathan, Self-calibration of asynchronized camera networks, in: Computer Vision Workshops (ICCV Workshops), 2009 IEEE
12th International Conference on, IEEE, 2009, pp. 2164\-2171.

 \bibitem{79} S. Dong, X. Shao, X. Kang, F. Yang, X. He, Extrinsic calibration of a
non-overlapping camera network based on close-range photogrammetry,
 Applied optics 55 (23) (2016) 6363\-6370.

 \bibitem{80} H. Hu, J. Liang, Z.-Z. Tang, B.-Q. Shi, X. Guo, Global calibration
for multi-camera videogrammetric system with large-scale field-of-view,
Guangxue Jingmi Gongcheng(Optics and Precision Engineering) 20 (2)
(2012) 369\-378.


 \bibitem{81} T. Birdal, E. Bala, T. Eren, S. Ilic, Online inspection of 3d parts via a
locally overlapping camera network, in: Applications of Computer Vision
(WACV), 2016 IEEE Winter Conference on, IEEE, 2016, pp. 1\-10.

 \bibitem{82} D. J. Cook, J. C. Augusto, V. R. Jakkula, Ambient intelligence: Technologies, applications, and opportunities, Pervasive and Mobile Computing
 5 (4) (2009) 277\-298.

 \bibitem{83} T. E. McSween, Values-based safety process: Improving your safety culture with behavior-based safety, John Wiley \& Sons, 2003.

 \bibitem{84} C. Fuller, An assessment of the relationship between behaviour and injury
in the workplace: A case study in professional football, Safety science
 43 (4) (2005) 213\-224.

 \bibitem{85} N. J. Bahr, System safety engineering and risk assessment: a practical
approach, CRC Press, 2014.

 \bibitem{86} T. Kongsvik, J. Fenstad, C. Wendelborg, Between a rock and a hard place:
Accident and near-miss reporting on offshore service vessels, Safety science
 50 (9) (2012) 1839\-1846.

 \bibitem{87} H. Li, M. Lu, S.-C. Hsu, M. Gray, T. Huang, Proactive behavior-based
safety management for construction safety improvement, Safety science
75 (2015) 107\-117.

 \bibitem{88} A. M. Shariff, N. Norazahar, At-risk behaviour analysis and improvement
 study in an academic laboratory, Safety science 50 (1) (2012) 29-38.

 \bibitem{89} C. Qing-gui, L. Kai, L. Ye-jiao, S. Qi-hua, Z. Jian, Risk management and
workers safety behavior control in coal mine, Safety science 50 (4) (2012)
909\-913.
 \bibitem{90} A. Laureshyn, Application of automated video analysis to road user behaviour, 2010.

\item \relax [91} T. Lv, H.-y. Zhang, C.-h. Yan, Double mode surveillance system based
on remote audio/video signals acquisition, Applied Acoustics 129 (2018)
316\-321.

 \bibitem{92} Y. Qu, T. Wang, Z. Zhu, Remote audio/video acquisition for human signa-
 ture detection, in: Computer Vision and Pattern Recognition Workshops,
2009. CVPR Workshops 2009. IEEE Computer Society Conference on,
IEEE, 2009, pp. 66\-71.

 \bibitem{93} H.-y. Zhang, T. Lv, C. Yan, The novel role of arctangent phase algorithm
and voice enhancement techniques in laser hearing, Applied Acoustics 126
 (2017) 136\-142.

 \bibitem{94} M. Kyriakidis, R. Hirsch, A. Majumdar, Metro railway safety: An analysis
of accident precursors, Safety science 50 (7) (2012) 1535\-1548.

 \bibitem{95} S. Andriulo, M. G. Gnoni, Measuring the effectiveness of a near-miss management system: An application in an automotive firm supplier, Reliability Engineering \& System Safety 132 (2014) 154\-162.

 \bibitem{96} S. C. Lubobya, M. E. Dlodlo, G. De Jager, A. Zulu, Throughput characteristics of wimax video surveillance systems, Procedia Computer Science
45 (2015) 571\-580.

 \bibitem{97} M.-J. Yang, J. Y. Tham, D. Wu, K. H. Goh, Cost effective ip camera
 for video surveillance, in: Industrial Electronics and Applications, 2009.
ICIEA 2009. 4th IEEE Conference on, IEEE, 2009, pp. 2432\-2435.

 \bibitem{98} B. Gumaidah, H. Soliman, Wimax network performance improvement
through the optimal use of available bandwidth by adaptive selective voice
coding, International Journal of Modern Engineering Sciences 2 (1) (2013)
1\-16.

 \bibitem{99} J. Changjiang, W. Jin, L. Mingfu, L. Zhichuan, A design and implementation of mobile video surveillance terminal base on arm, Procedia Computer
Science 107 (2017) 498\-502.

 \bibitem{100} N. Chen, Y. Chen, Y. You, H. Ling, P. Liang, R. Zimmermann, Dynamic
urban surveillance video stream processing using fog computing, in: Mul-
53timedia Big Data (BigMM), 2016 IEEE Second International Conference
on, IEEE, 2016, pp. 105\-112.

 \bibitem{101} D. A. Rodr´ıguez-Silva, L. Adkinson-Orellana, F. Gonz’lez-Castano,
I. Armino-Franco, D. Gonz’lez-Martinez, Video surveillance based on
 cloud storage, in: Cloud Computing (CLOUD), 2012 IEEE 5th International Conference on, IEEE, 2012, pp. 991\-992.

 \bibitem{102} N. Chen, Y. Chen, S. Song, C.-T. Huang, X. Ye, Smart urban surveillance
using fog computing, in: Edge Computing (SEC), IEEE/ACM Symposium on, IEEE, 2016, pp. 95\-96.

 \bibitem{103} H. Sun, X. Liang, W. Shi, Vu: video usefulness and its application in largescale video surveillance systems: an early experience, in: Proceedings of
the Workshop on Smart Internet of Things, ACM, 2017, p. 6.

 \bibitem{104} Q. Zhang, Z. Yu, W. Shi, H. Zhong, Demo abstract: Evaps: Edge video
analysis for public safety, in: Edge Computing (SEC), IEEE/ACM Symposium on, IEEE, 2016, pp. 121\-122.

 \bibitem{105} R. Du, S. Bista, A. Varshney, Video fields: fusing multiple surveillance
videos into a dynamic virtual environment, in: Proceedings of the 21st
International Conference on Web3D Technology, ACM, 2016, pp. 165\-172.

 \bibitem{106} S. Singh, C. Shekhar, A. Vohra, Fpga-based real-time motion detection
for automated video surveillance systems, Electronics 5 (1) (2016) 10.

 \bibitem{107} Y. Li, R. Xia, Q. Huang, W. Xie, X. Li, Survey of spatio-temporal interest
point detection algorithms in video, IEEE Access 5 (2017) 10323\-10331.

 \bibitem{108} B. Tian, B. T. Morris, M. Tang, Y. Liu, Y. Yao, C. Gou, D. Shen, S. Tang,
 Hierarchical and networked vehicle surveillance in its: A survey, IEEE
Transactions on Intelligent Transportation Systems 18 (1) (2017) 25-48.

 \bibitem{109} T. Bouwmans, A. Sobral, S. Javed, S. K. Jung, E.-H. Zahzah, Decomposition into low-rank plus additive matrices for background/foreground separation: A review for a comparative evaluation with a large-scale dataset,
Computer Science Review 23 (2017) 1-71.

 \bibitem{110} O. Elharrouss, A. Abbad, D. Moujahid, H. Tairi, Moving object detection
zone using a block-based background model, IET Computer Vision 12 (1)
(2017) 86-94.

 \bibitem{111} O. Elharrouss, D. Moujahid, S. Elkah, H. Tairi, Moving object detection
 using a background modeling based on entropy theory and quad-tree decomposition, Journal of Electronic Imaging 25 (6) (2016) 061615.

 \bibitem{112} E. Cerme~no, A. P´erez, J. A. Sig¨uenza, Intelligent video surveillance beyond robust background modeling, Expert Systems with Applications 91
(2018) 138-149.

 \bibitem{113} F.-C. Cheng, S.-C. Huang, S.-J. Ruan, Illumination-sensitive background
modeling approach for accurate moving object detection, IEEE Transactions on broadcasting 57 (4) (2011) 794-801.

 \bibitem{114} Y. Wang, Q. Lu, D. Wang, W. Liu, Compressive background modeling for
foreground extraction, Journal of Electrical and Computer Engineering
2015 (2015) 13.

 \bibitem{115} B.-H. Chen, S.-C. Huang, J.-Y. Yen, Counter-propagation artificial neural
network-based motion detection algorithm for static-camera surveillance
scenarios, Neurocomputing 273 (2018) 481-493.

 \bibitem{116} W. Bouachir, R. Noumeir, Automated video surveillance for preventing
suicide attempts.

 \bibitem{117} W. Bouachir, R. Gouiaa, B. Li, R. Noumeir, Intelligent video surveillance
for real-time detection of suicide attempts, Pattern Recognition Letters
110 (2018) 1-7.

 \bibitem{118} R. Kachach, J. M. Ca~nas, Hybrid three-dimensional and support vector
machine approach for automatic vehicle tracking and classification using
a single camera, Journal of Electronic Imaging 25 (3) (2016) 033021.

 \bibitem{119} Y. Dedeo˘glu, B. U. T¨oreyin, U. Gudukbay, A. E. C¸ etin, Silhouette-based
method for object classification and human action recognition in video,
in: European Conference on Computer Vision, Springer, 2006, pp. 64-77.

 \bibitem{120} F. Wu, X.-Y. Jing, X. You, D. Yue, R. Hu, J.-Y. Yang, Multi-view lowrank dictionary learning for image classification, Pattern Recognition 50
(2016) 143-154.


 \bibitem{121} M. Imani, H. Ghassemian, Edge-preserving-based collaborative representation for spectral-spatial classification, International Journal of Remote
 Sensing 38 (20) (2017) 5524-5545.

 \bibitem{122} Y. Gurwicz, R. Yehezkel, B. Lachover, Multiclass object classification for
real-time video surveillance systems, Pattern Recognition Letters 32 (6)
(2011) 805-815.

 \bibitem{123} N. Najva, K. E. Bijoy, Sift and tensor based object detection and classification in videos using deep neural networks, Procedia Computer Science
93 (2016) 351-358.

 \bibitem{124} M. U. Yaseen, A. Anjum, O. Rana, R. Hill, Cloud-based scalable object
detection and classification in video streams, Future Generation Computer
Systems 80 (2018) 286-298.

 \bibitem{125} I. Elafi, M. Jedra, N. Zahid, Unsupervised detection and tracking of moving objects for video surveillance applications, Pattern Recognition Letters
84 (2016) 70-77.

 \bibitem{126} X. Li, W. Hu, C. Shen, Z. Zhang, A. Dick, A. V. D. Hengel, A survey of
appearance models in visual object tracking, ACM transactions on Intelligent Systems and Technology (TIST) 4 (4) (2013) 58.

 \bibitem{127} D. Moujahid, O. Elharrouss, H. Tairi, Visual object tracking via the local
soft cosine similarity, Pattern Recognition Letters 110 (2018) 79-85.

 \bibitem{128} D. Moujahid, O. Elharrouss, H. Tairi, Visual moving object tracking via
sparse representation based trackers: A comparative study, in: Complex
Systems (WCCS), 2015 Third World Conference on, IEEE, 2015, pp. 1-6.

 \bibitem{129} A. W. Smeulders, D. M. Chu, R. Cucchiara, S. Calderara, A. Dehghan,
M. Shah, Visual tracking: An experimental survey, IEEE transactions on
pattern analysis and machine intelligence 36 (7) (2014) 1442-1468.

 \bibitem{130} Z. Kalal, K. Mikolajczyk, J. Matas, Tracking-learning-detection, IEEE
 transactions on pattern analysis and machine intelligence 34 (7) (2012)
1409-1422.

 \bibitem{131} B. Zhuang, H. Lu, Z. Xiao, D. Wang, Visual tracking via discriminative
sparse similarity map, IEEE Transactions on Image Processing 23 (4)
(2014) 1872-1881.

 \bibitem{132} X. Cheng, N. Li, T. Zhou, L. Zhou, Z. Wu, Object tracking via collaborative multi-task learning and appearance model updating, Applied Soft
Computing 31 (2015) 81-90.

 \bibitem{133} W. Zhong, H. Lu, M.-H. Yang, Robust object tracking via sparse collaborative appearance model, IEEE Transactions on Image Processing 23 (5)
 (2014) 2356-2368.

 \bibitem{134} S. Murthy, B. Sujatha, Multi-level optimization in encoding to balance
video compression and retention of 8k resolution, Perspectives in Science
8 (2016) 338-344.

 \bibitem{135} N. Patil, S. Ambatkar, S. Kakde, Iot based smart surveillance security
system using raspberry pi, in: Communication and Signal Processing
(ICCSP), 2017 International Conference on, IEEE, 2017, pp. 0344-0348.

 \bibitem{136} D. Minoli, K. Sohraby, B. Occhiogrosso, Iot considerations, requirements, and architectures for smart buildingsenergy optimization and nextgeneration building management systems, IEEE Internet of Things Journal 4 (1) (2017) 269-283.

 \bibitem{137} A. Khan, B. Rinner, A. Cavallaro, Cooperative robots to observe moving
targets, IEEE transactions on cybernetics.

 \bibitem{138} S. Zhu, Z. Xu, Spatiotemporal visual saliency guided perceptual high efficiency video coding with neural network, Neurocomputing 275 (2018)
 511-522.

 \bibitem{139} J. Galan-Hernandez, V. Alarcon-Aquino, O. Starostenko, J. RamirezCortes, P. Gomez-Gil, Wavelet-based frame video coding algorithms using fovea and speck, Engineering Applications of Artificial Intelligence 69
(2018) 127-136.

 \bibitem{140} N. Chen, Y. Chen, X. Ye, H. Ling, S. Song, C.-T. Huang, Smart city
surveillance in fog computing, in: Advances in Mobile Cloud Computing
and Big Data in the 5G Era, Springer, 2017, pp. 203-226.

 \bibitem{141} A. J. Neto, Z. Zhao, J. J. Rodrigues, H. B. Camboim, T. Braun, Fogbased crime-assistance in smart iot transportation system, IEEE Access
6 (2018) 11101-11111.

 \bibitem{142} S. Chen, T. Zhang, W. Shi, Fog computing, IEEE Internet Computing
21 (2) (2017) 4-6.

 \bibitem{143} X. Yue, Y. Liu, J. Wang, H. Song, H. Cao, Software defined radio and
wireless acoustic networking for amateur drone surveillance, IEEE Com-
 munications Magazine 56 (4) (2018) 90-97.

 \bibitem{144} S. Baidya, M. Levorato, Content-aware cognitive interference control for
urban iot systems, IEEE Transactions on Cognitive Communications and
Networking.


\end{thebibliography}

